Switching Controller Synthesis for Hybrid Systems Against STL Formulas

Switching controllers play a pivotal role in directing hybrid systems (HSs) towards the desired objective, embodying a ``correct-by-construction'' approach to HS design. Identifying these objectives is thus crucial for the synthesis of effective switching controllers. While most of existing works focus on safety and liveness, few of them consider timing constraints. In this paper, we delves into the synthesis of switching controllers for HSs that meet system objectives given by a fragment of STL, which essentially corresponds to a reach-avoid problem with timing constraints. Our approach involves iteratively computing the state sets that can be driven to satisfy the reach-avoid specification with timing constraints. This technique supports to create switching controllers for both constant and non-constant HSs. We validate our method's soundness, and confirm its relative completeness for a certain subclass of HSs. Experiment results affirms the efficacy of our approach.

==> macros.tex <==
\RequirePackage[disable]{todonotes}

% Todonotes
\newcommand{\sfcomment}[1]{\todo[color=NavyBlue!30,size=\small,fancyline,author=Shenghua]{#1}\xspace}

\newcommand{\haocomment}[1]{\todo[color=Yellow!30,size=\small,fancyline,author=HaoWu]{#1}\xspace}

\newcommand{\simoncomment}[1]{\todo[color=Orange!30,size=\small,fancyline,author=Simon]{#1}\xspace}

\newcommand{\sfcommentinline}[1]{\todo[inline,color=NavyBlue!30,author=Shenghua]{#1}\xspace}
\newcommand{\atsf}{\colorbox{NavyBlue!30}{\textbf{@Shenghua}}}

\newcommand{\oomit}[1]{}

\newcommand{\reviewercomment}[1]{\todo[color=RedViolet!30,size=\small,fancyline,author=Reviewer]{#1}\xspace}

\newcommand{\hscomment}[1]{\todo[color=SeaGreen!60,size=\small,fancyline,author=Han]{#1}\xspace}
\newcommand{\hscommentinline}[1]{\todo[inline,color=SeaGreen!60,author=Han]{#1}\xspace}
\newcommand{\aths}{\colorbox{SeaGreen!60}{\textbf{@Han}}}


\newcommand{\nzcomment}[1]{\todo[color=Orange!30,size=\small,fancyline,author=Naijun]{#1}\xspace}
\newcommand{\nzcommentinline}[1]{\todo[inline,color=Orange!30,author=Naijun]{#1}\xspace}
\newcommand{\atnz}{\colorbox{Orange!30}{\textbf{@Naijun}}}

%Colors
\definecolor{myred}{HTML}{e41a1c}
\definecolor{myblue}{HTML}{377eb8}
\definecolor{mygreen}{HTML}{4daf4a}
\definecolor{mygray}{gray}{0.6}
\definecolor{myorange}{HTML}{ffa510}
\newcommand{\green}[1]{\textcolor{mygreen}{#1}}
\newcommand{\red}[1]{\textcolor{myred}{#1}}
\newcommand{\blue}[1]{\textcolor{myblue}{#1}}
\newcommand{\violet}[1]{\textcolor{RedViolet}{#1}}
\newcommand{\orange}[1]{\textcolor{myorange}{#1}}
\newcommand{\gray}[1]{\textcolor{mygray}{#1}} 

% Real, Natural ...
\newcommand{\Reals}{\mathbb{R}\xspace}
\newcommand{\PosReals}{\mathbb{R}_{> 0}\xspace}
\newcommand{\NonNegReals}{\mathbb{R}_{\ge 0}\xspace}
\newcommand{\Realn}{\mathbb{R}^n\xspace}
\newcommand{\Nats}{\mathbb{N}\xspace}
\newcommand{\PosNats}{\mathbb{N}_{>0}\xspace}
\newcommand{\Ints}{\mathbb{Z}\xspace}

% Vectors
\newcommand{\ff}{\bm{f}\xspace}
\newcommand{\xx}{\bm{x}\xspace}
\newcommand{\yy}{\bm{y}\xspace}
\newcommand{\uu}{\bm{u}\xspace}
\newcommand{\fa}{\bm{a}\xspace}
\newcommand{\fb}{\bm{b}\xspace}
\newcommand{\xxi}{\bm{\xi}\xspace}

% \llangle for [[, \rragnel for ]]
\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1[}\)}%
  \mathopen{\copy\@brx\kern-0.6\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1]}\)}%
  \mathclose{\copy\@brx\kern-0.6\wd\@brx\usebox{\@brx}}}
\makeatother

% Hybrid Automaton 
\newcommand{\HyAuto}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\ContiState}{\ensuremath{X}\xspace}
\newcommand{\DisState}{\ensuremath{Q}\xspace}
\newcommand{\Edge}{\ensuremath{E}\xspace}
\newcommand{\Init}[1][]{\ensuremath{\mathtt{Init}\ifthenelse{\equal{#1}{}}{}{(#1)}}\xspace}
\newcommand{\Inv}[1][]{\ensuremath{\mathtt{Inv}\ifthenelse{\equal{#1}{}}{}{(#1)}}\xspace}
\newcommand{\Flow}[1][]{\ensuremath{\mathtt{Flow}\ifthenelse{\equal{#1}{}}{}{(#1)}}\xspace}
\newcommand{\Jump}[1][]{\ensuremath{\mathtt{Jump}\ifthenelse{\equal{#1}{}}{}{(#1)}}\xspace}
\newcommand{\tJump}[1][]{\ensuremath{\mathtt{Jump}_t\ifthenelse{\equal{#1}{}}{}{(#1)}}\xspace}
\newcommand{\Dom}[1][]{\ensuremath{\mathtt{Dom}\ifthenelse{\equal{#1}{}}{}{(#1)}}\xspace}
\newcommand{\post}[1]{\ensuremath{\mathtt{Post}(#1)}\xspace}
\newcommand{\pre}[1]{\ensuremath{\mathtt{Pre}(#1)}\xspace}

\newcommand{\Traj}[1][]{\ensuremath{\xx\ifthenelse{\equal{#1}{}}{}{(#1)}}\xspace}
\newcommand{\dTraj}[1][]{\ensuremath{\dot{\xx}\ifthenelse{\equal{#1}{}}{}{(#1)}}\xspace}
\newcommand{\pTraj}[1][]{\ensuremath{\xx'\ifthenelse{\equal{#1}{}}{}{(#1)}}\xspace}
\newcommand{\Reach}{\ensuremath{\mathtt{Reach}}\xspace}
\newcommand{\Seman}[1]{\ensuremath{\llangle #1 \rrangle}\xspace}

% Symble
\newcommand{\repl}{\!=\!}
\newcommand{\Def}{\mathrel{::=}}
\newcommand{\LogiEq}{\leftrightarrow}
\makeatletter
\newcommand{\Pminus}{\mathbin{\mathpalette\prc@inner\relax}} % over-dotted minus
\newcommand{\prc@inner}[2]{%
  \vbox{\offinterlineskip\m@th
    \ialign{%
      ##\cr
      \hidewidth\raisebox{-1.5\height}[0pt][0pt]{$#1.$}\hidewidth\cr
      $#1-$\cr
    }%
  }%
}
\makeatother
\newcommand{\qe}{\ensuremath{\mathtt{QE}}\xspace}
\newcommand{\fp}{\scriptsize{(\textsf{fp})}}
\newcommand{\mcheck}{\usym{1F5F8}}
\newcommand{\mtimes}{\scriptsize{\usym{2613}}}

%STL temporal operator
\newcommand{\until}[1][]{\ensuremath{\,\mathcal{U}\ifthenelse{\equal{#1}{}}{}{\ifthenelse{\pdfmatch{,}{#1}=1}{_{[#1]}}{_{#1}}}}\xspace}
\newcommand{\always}[1][]{\ensuremath{\Box\ifthenelse{\equal{#1}{}}{}{\ifthenelse{\pdfmatch{,}{#1}=1}{_{[#1]}}{_{#1}}}}\xspace}
\newcommand{\eventually}[1][]{\ensuremath{\Diamond\ifthenelse{\equal{#1}{}}{}{\ifthenelse{\pdfmatch{,}{#1}=1}{_{[#1]}}{_{#1}}}}\xspace}
\newcommand{\fr}[1]{\ensuremath{fr(#1)}\xspace}
\newcommand{\tts}[2]{\ensuremath{ts({#1},{#2})}\xspace}
\newcommand{\ffs}[2]{\ensuremath{fs({#1},{#2})}\xspace}

% Guard Condition Synthesize
\newcommand{\lb}[1]{\ensuremath{lb_{#1}}\xspace}
\newcommand{\ub}[1]{\ensuremath{ub_{#1}}\xspace}




%%%%    Standards    %%%%

\newcommand{\mydot}{\text{{\Large\textbf{.}}~}}
\DeclareMathOperator{\dif}{\,d\!}
\newcommand{\stag}[1]{{\tag*{\small{({#1})}}}}
\newcommand{\TAG}[1]{{\tag*{\small{[{#1}]}}}}
\newcommand*\from{\colon}
\newcommand{\supp}{\mathtt{supp}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

%%%%    Shortcuts    %%%%

\newcommand{\minimize}{\mathtt{minimize}}
\newcommand{\subj}{\mathtt{subject~to}}


\newcommand{\tiff}{\textnormal{iff}\quad}
\newcommand{\qiff}{\ \quad\textnormal{iff}\quad\ }
\newcommand{\qqiff}{\qquad\textnormal{iff}\qquad}
\newcommand{\lqiff}{\textnormal{iff}\quad}
\newcommand{\lqqiff}{\textnormal{iff}\qquad}

\newcommand{\aand}{\ \ \textnormal{and}\ \ }
\newcommand{\qand}{\ \quad\textnormal{and}\quad\ }
\newcommand{\qqand}{\qquad\textnormal{and}\qquad}

\newcommand{\oor}{\ \ \textnormal{or}\ \ }
\newcommand{\qor}{\ \quad\textnormal{or}\quad\ }
\newcommand{\qqor}{\qquad\textnormal{or}\qquad}

\newcommand{\ffor}{\ \ \textnormal{for}\ \ }
\newcommand{\fforany}{\ \ \textnormal{for any}\ \ }
\newcommand{\qfor}{\ \quad\textnormal{for}\quad\ }
\newcommand{\qqfor}{\qquad\textnormal{for}\qquad}

\newcommand{\wwith}{\ \ \textnormal{with}\ \ }
\newcommand{\qwith}{\ \quad\textnormal{with}\quad\ }
\newcommand{\qqwith}{\qquad\textnormal{with}\qquad}

\newcommand{\qimplies}{\ \quad\textnormal{implies}\quad\ }
\newcommand{\qqimplies}{\qquad\textnormal{implies}\qquad}
\newcommand{\lqimplies}{\textnormal{implies}\quad}
\newcommand{\lqqimplies}{\textnormal{implies}\qquad}

\newcommand{\pprec}{\mathrel{{\prec}\hspace{-.5ex}{\prec}}}
\newcommand{\ppprec}{~{}\pprec{}~}
\newcommand{\npprec}{\centernot\pprec}

\newcommand{\ppreceq}{~{}\preceq{}~}
\newcommand{\ssucceq}{~{}\succeq{}~}
\newcommand{\defeq}{{}\triangleq{}}
\newcommand{\define}{\defeq}
\newcommand{\ddefeq}{\ {}\defeq{}\ }
\newcommand{\eeq}{~{}={}~}
\newcommand{\mmapsto}{~{}\mapsto{}~}
\newcommand{\eequiv}{~{}\equiv{}~}
\newcommand{\pplus}{~{}+{}~}
\newcommand{\ccdot}{~{}\cdot{}~}
\newcommand{\llongrightarrow}{~{}\longrightarrow{}~}
\newcommand{\qlongrightarrow}{\quad{}\longrightarrow{}\quad}
\newcommand{\qqlongrightarrow}{\qquad{}\longrightarrow{}\qquad}
\newcommand{\mmid}{~{}\mid{}~}
\newcommand{\qmid}{\quad{}|{}\quad}
\newcommand{\tto}{~{}\to{}~}
\newcommand{\uuplus}{\,{}\uplus{}\,}
\newcommand{\nneq}{~{}\neq{}~}
\newcommand{\qeq}{\quad{}={}\quad}
\newcommand{\qqeq}{\qquad{}={}\qquad}
\newcommand{\lleq}{~{}\leq{}~}
\newcommand{\LL}{~{}<{}~}
\newcommand{\GG}{~{}>{}~}
\newcommand{\ggeq}{~{}\geq{}~}
\newcommand{\ssqsubseteq}{~{}\sqsubseteq{}~}
\newcommand{\iimplies}{~{}\implies{}~}
\newcommand{\mmodels}{~{}\models{}~}
\newcommand{\nnotmodels}{~{}\not\models{}~}
\newcommand{\iin}{~{}\in{}~}
\newcommand{\nnotin}{~{}\not\in{}~}
\newcommand{\wwedge}{~{}\wedge{}~}
\newcommand{\vvee}{~{}\vee{}~}

\newcommand{\cwedge}{\,{}\wedge{}\,}

%Colorful equation
% Commands for Highlighting text -- non tikz method
%\newcommand{\highlight}[2]{\colorbox{#1!17}{$\displaystyle #2$}}
%\newcommand{\highlight}[2]{\colorbox{#1!17}{$#2$}}

% Commands for Highlighting text -- non tikz method
%\renewcommand{\highlight}[2]{\colorbox{#1!17}{#2}}




%for qedT mark compatible within displaymath
\def\triangleforqed{\hbox{$\lhd$}}
\makeatletter
\DeclareRobustCommand{\qedT}{%
	\ifmmode
	\eqno \def\@badmath{$$}%$$
	\let\eqno\relax \let\leqno\relax \let\veqno\relax
	\hbox{\triangleforqed}%
	\else
	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
	\quad\hbox{\triangleforqed}%
	\fi
}
\makeatother

==> sections/sec_switchautomata.tex <==

\section{Synthesis of Switched Hybrid Automata}\label{sec:state-dep}
\hscommentinline{Simplify this section}
%    In this section, we will give a method to synthesize switched hybrid automaton, based on the time-relevant guard conditions $\{G_t(e)^i\}_{i=0}^k$ and the initial set $\{\Init[q]^i\}_{i=0}^k$ calculated in \cref{sec:prob1}.
    %we try to synthesize new switching conditions such that all the trajectories following the new jump conditions will satisfy the STL specification $\varphi$ in this subsection.

    In this section, we consider the state-dependent switching controller synthesis problem, which aims to synthesize a switched hybrid automata. 
    This task is notably challenging~\cite{henzinger1995s}.
    To tackle this, we introduce an effective method to synthesize switched hybrid automata with \emph{constant dynamics}, leveraging the state-time sets $\{X_q^i\}_{q\in Q}$ and the initial set $\{\Init[q]^i\}_{q\in Q}$ calculated in \cref{sec:prob1}.

    The synthesis of switched hybrid automata requires a predefined discrete transition set $E$ between modes, as detailed in the problem formulation of \cref{para:prob_form}
    %\simoncomment{need a ref back to the previous section}. 
    For time-dependent switching controllers discussed in \cref{sec:prob1}, this set is essentially $Q\times Q\setminus \{(q,q)\mid q\in Q\}$. Limiting $E$ to a subset of this representation maintains our method's soundness. Therefore, by incorporating the discrete transition set $E$ into \cref{alg:time-relevant-syn}, specifically by changing $\vee_{q'\neq q}$ to $\vee_{(q,q')\in E}$ in \cref{eq:X_q^i}, the state-time sets $\{X_q^i\}_{q\in Q}$ we get can serve as a viable guard conditions on both state $x$ and time $t$. However, these conditions, being time-relevant, do not align with the semantics of switched hybrid automata. To resolve this, we introduce a method to eliminate the time variable $t$ in $X_q^i$ while ensuring the inclusion of a broad spectrum of initial conditions.

%    The synthesis of switched hybrid automata require a given discrete transition $E$ between modes (see \cref{subsec:prob}). The discrete transition when considering time-dependent switching controller essentially can be seen as $Q\times Q$, and constrain the discrete transition $E$ to a subset of $Q\times Q$ will not influence the soundness and correctness of our method. Therefore, by encoding the discrete transition $E$ of switched hybrid automata into \cref{alg:time-relevant-syn} — that is, adding a justification for whether $(q,q')\in E$ following line \ref{alg1:for-loop} in \cref{alg:time-relevant-syn} — we successfully establish feasible guard conditions considering both state $x$ and time $t$. However, these time-relevant guard conditions do not comply with the semantics of switched hybrid automata. Therefore, we propose a method to eliminate the time $t$ in $G_t(e)^i$ and ensure the inclusion of a comprehensive range of initial conditions.

    \subsection{Eliminating $t$ in State-Time Set}
    %To eliminate $t$ in $X_q^i$, 
    We first introduce the concept of \emph{time-relevant reachable set}. 
    \begin{definition}
        For a set $K$ defined by state $x$ and time $t$, the time-relevant reachable set of differential dynamics governed by $\dot\xx = f(\xx)$ is 
        \begin{align}
            %\Reach(K) \defeq \{ (\xx(\tau;x,t),\tau) \mid \xx\in\Seman{f}, \tau\ge t, (x,t)\in K\},\\
            \Reach(K) \defeq \{ (x,\tau) \mid \tau\ge t_0, x=\Psi(\tau;x_0,t_0), (x_0,t_0)\in K\}, \label{eq:def-reach}
        \end{align}
        where $\Psi(\,\cdot\,;x_0,t_0)$ represents the solution of $\dot\xx = f(\xx)$ initiating from point $x_0$ at time $t_0$.
    \end{definition}
    
    As we considered constant dynamics in this section, the following theorem provides an exact characterization of the time-relevant reachable set for the differential dynamics governed by $\dot \xx = a$.
\begin{restatable}{theorem}
    {restateTReach}\label{thm:t-reach}
        For a given set $K$ with the corresponding flow condition $\dot \xx = a$,
        \begin{align}\label{eq:reachable-set}
            \Reach(K) = \qe\left(\exists \delta\ge 0,~ K[x,t\repl x - \delta a,t - \delta]\right)
        \end{align}
\end{restatable}
\oomit{    \begin{proof}
        Let $\tau - t_0 = \delta$ in \cref{eq:def-reach}, then for the differential dynamics governed by $\dot\xx = a$,
        \begin{align*}
            \Reach(K) & = \{ (x,\tau) \mid \delta\ge 0, x = x_0 + \delta a, \tau = t_0 + \delta, (x_0,t_0)\in K \}\\
                      & = \{ (x,\tau) \mid \delta \ge 0, (x-\delta a, \tau-\delta) \in K \}.
        \end{align*}
        Thus, $(x,\tau)\in\Reach(K)$ iff $\exists \delta\ge 0,~ (x,\tau)\in K[x,t\repl x-\delta a,t-\delta]$
        \qed
    \end{proof} }

    For the initial set $\{\Init[q]^i\}_{q\in Q}$ calculated in \cref{alg:time-relevant-syn}, %where the time variable $t$ is replaced by $0$, the reachable set 
    its time-relevant reachable set can be calculated by substituting $K = \Init[q]^i\wedge(t=0)$ into \cref{eq:reachable-set}. For ease of notation, we use $\Reach(\Init[q]^i)$ to represents $\Reach(\Init[q]^i\wedge(t=0))$.
    %The reason for defining the time-relevant reachable set here is that, during the procedure of eliminating $t$ in $\{X_q^i\}_{i=0}^k$, we need to calculate the reachable set from some intermediate sets where $t\neq 0$, as illustrated in \cref{exp:WTS-conflict}.

    We now define the \emph{$i$-switches guard condition} derived from $X_q^i$ by eliminating the time variable $t$.

    \begin{definition}\label{def:t-eliminate}
        For a given index $i\in\Nats$, consider the initial set $\Init[q]^{i+1}$ and the state-time set $X_{q'}^i$, where $(q,q')\in E$. The state set $G(q,q')^i$ is defined as the $i$-switches guard condition relative to $X_{q'}^{i}$ and $\Init[q]^{i+1}$ if it fulfills the following criterion:
        \begin{align}\label{eq:t-irr-formula}
            \forall (x,\tau),~(x,\tau)\in \left(\Reach(\Init[q]^{i+1})\wedge G(q,q')^i\right)\implies (x,\tau)\in X_{q'}^i
        \end{align}  
    \end{definition}

    $G(q,q')^i$ is a set of states ensuring that if a trajectory transitions from $q$ to $q'$ while within $G(q,q')^i$, it can satisfy the specified ST-RA formula $\varphi$ within additional $i$ times of transitions. To satisfy this, $G(q,q')^i$ must ensure that any execution starting from $\Init[q]^{i+1}$ remains within $G(q,q')^i$ (i.e., $(x,\tau)\in\Reach(\Init[q]^{i+1})\wedge G(q,q')^i$) should also be in $X_{q'}^i$ (i.e., $(x,\tau)\in X_{q'}^i$). The following example gives an illustrative explanation of $i$-switches guard conditions.

%    Intuitively, to effectively eliminate the time variable $t$ in $X_{q'}^i$ while adhering to the ST-RA formula $\varphi$, it is essential that the executions originating from the initial set $\Init[q]^{i+1}$ that meeting the $t$-elimination guard condition $G(q,q')^i$ (i.e., $(x,\tau)\in\Reach(\Init[q]^i)\wedge G(q,q')^i$) must also fulfill the 
%   
%    (i.e., $(x,\tau)\in X_{q'}^i$). The following example gives an illustrative explanation of $t$-eliminated guard conditions.
    \begin{example}\label{exp:WTS-guard}
        Building upon \cref{exp:alg1-resul}, we assume that the initial condition for 
        {\makeatletter
        \let\par\@@par
        \par\parshape0
        \everypar{}
        \begin{wrapfigure}{r}{0.42\textwidth}
		    \centering
            \vspace{-0.85cm}
            \begin{adjustbox}{max width = 1\linewidth}
		        \begin{tikzpicture}[font=\scriptsize]
		            \begin{groupplot}[ Axis Set, height = 3.6cm, group style={group size = 1 by 1, horizontal sep = 0.5cm}]
		                %%%X_{q_1}^1
                        \nextgroupplot[xmax=5, ymax=5.5,xlabel=$t$,ylabel=$h$,ytick={1,1.5,2,3,4,5}]
                        \addplot[name path = X1, draw = none] (0.7,0.7) node {$X_{q_1}^0$};
                        \addplot[name path = G1U, domain = {0:1}, draw = none] {x+1};
                        \addplot[name path = G1L, domain = {0:1}, draw = none] {0};
                        \addplot[fill=myorange!20]fill between[of=G1U and G1L, soft clip={domain=0:1}];
                        \addplot[name path = G2U, domain = {1:3}, draw = none] {x+1};
                        \addplot[name path = G2L, domain = {1:3}, draw = none] {x-1};
                        \addplot[fill=myorange!20]fill between[of=G2U and G2L, soft clip={domain=1:3}];
                        \addplot[name path = G3U, domain = {3:4}, draw = none] {4};
                        \addplot[name path = G3L, domain = {3:4}, draw = none] {x-1};
                        \addplot[fill=myorange!20]fill between[of=G3U and G3L, soft clip={domain=3:4}];
                        % Reachable set from [3,4]
                        \node[coordinate, pin={[pin edge={Black}]60:{{$\Reach(\Init[q_2]^1)$}}}] at (axis cs:0.4, 3){};
                        \addplot[name path = reach3, domain = {0:3}, color = mygreen, thick] {-x+3};
                        \addplot[name path = reach4, domain = {0:3}, color = mygreen, thick] {-x+4};
                        % t-eleminate result
                        \addplot[name path = guardUB, domain = {0:3}, color = mygray, thick] {2};
                        \addplot[name path = guardLB, domain = {0:3}, color = mygray, thick] {1.5};
                        
                        % The STL specification
		                \addplot[name path = Phi2Up,  domain = {3:4}, color=myblue] {5}; % node [right] {$\phi_2$};
		                \addplot[name path = Phi2Low, domain = {3:4}, color=myblue] {3};
                        \addplot[name path = Phi1, domain = {0:4}, color = myred] {4}; % node [right] {$\phi_1$};
                        % Dash line
		                \draw[dashed] ($(axis cs:3,\pgfkeysvalueof{/pgfplots/ymax})!{1/11}!(axis cs:3,\pgfkeysvalueof{/pgfplots/ymin})$) -- (axis cs:3,\pgfkeysvalueof{/pgfplots/ymin});
		                \draw[dashed] ($(axis cs:4,\pgfkeysvalueof{/pgfplots/ymax})!{1/11}!(axis cs:4,\pgfkeysvalueof{/pgfplots/ymin})$) -- (axis cs:4,\pgfkeysvalueof{/pgfplots/ymin});

                    \end{groupplot}
		        \end{tikzpicture}
            \end{adjustbox}
            \vspace{-0.7cm}
            \caption{Derive $G(q_2,q_1)^0$ from $X_{q_2}^0$}
            \label{fig:t-eliminate}
            \end{wrapfigure}
            \noindent
            control mode $q_1$ is confined to the interval $[0,3]$, and for $q_2$, it is limited to $[3,5]$. As depicted in \cref{fig:t-eliminate}, consider the initial set $\Init[q_2]^1 =[3,4]$. A $0$-switch guard condition, resulting from the elimination of $t$ in $X_{q_1}^0$, is $G(q_2,q_1)^0 = (1.5\le h\le 2)$
            %\simoncomment{double check this, should be 1.5?}\hscomment{Yes, corrected it}. 
            This condition complies with \cref{eq:t-irr-formula} as outlined in \cref{def:t-eliminate}, which is demonstrated as follows:

%            condition of control mode $q_1$ is restricted to the interval $[0,3]$, while the initial condition of $q_2$ is restricted to $[3,5]$. As illustrated in \cref{fig:t-eliminate}, for the initial set $\Init[q_2]^1=[3,4]$, one of the $0$-switches guard conditions derived from eliminate $t$ of $X_{q_1}^0$ is $G(q_2,q_1)^1 = (1.5 \leq h \leq 2)$, which satisfying \cref{eq:t-irr-formula} in \cref{def:t-eliminate} as below:
            
            \par}%
             \noindent
             
            \begin{align}\label{eq:eliminate-exp}
                \forall (x,\tau),~(x,\tau)\!\in\!\underbrace{\tikzmarknode{reach}{\green{\Reach(\Init[q_2]^1)}}\!\wedge\!\tikzmarknode{G}{\gray{(1.5\le h\le 2)}}}_{
                    \tikzmarknode{notation}{\substack{\text{\footnotesize{The intersection of region in}}\\ 
                    \text{ \footnotesize{``\qquad'' and ``\qquad''. }}}
                }}\! \implies\! (x,\tau)\!\in\!\colorbox{myorange!20}{$X_{q_1}^0$}
            \end{align}
            \begin{tikzpicture}[overlay,remember picture,>=stealth,nodes={align=left,inner ysep=1pt}]
            %    \draw [color = mygreen, line width=0.15mm] (reach.north) -| (reach.east) |- (reach.south) -| (reach.west) |- (reach.north) -- cycle;
            %    \draw [color = mygray, line width = 0.15mm] (G.north) -| (G.east) |- (G.south) -| (G.west) |- (G.north) -- cycle;
                \node (gren) [below of = notation, xshift=-1.25cm , yshift=1cm ] {};
                \node (gren1) [below of = gren, yshift=0.85cm] {};
                \draw [color = mygreen, thick] (gren) -- +(0.5,-0.18);
                \draw [color = mygreen, thick] (gren1) -- +(0.5,-0.18);

                \node (gray) [below of = notation, xshift=0.5cm , yshift=0.85cm ] {};
                \node (gray1) [below of = gray, yshift=0.85cm] {};
                \draw [color = mygray, thick] (gray) -- +(0.5,0);
                \draw [color = mygray, thick] (gray1) -- +(0.5,0);
            \end{tikzpicture}
%        \qedT
    \end{example}
    
    In the case of switched hybrid automata with constant dynamics, \cref{eq:t-irr-formula} can be efficiently resolved using quantifier elimination tools \cite{de2008z3}. However, as we will explore in the subsequent section, merely eliminating the time variable $t$ without accounting for the interrelations among various $i$-switches guard conditions for the same edge could result in vacuous guard conditions for the hybrid automata.

%        define the lower and upper bound of time-irrelevant jump condition in single dimension as below 
%        \begin{definition}
%            For a given dimension $x_j\in\ContiState$, the lower and upper bound of the time-relevant jump conditions with respect to the time-relevant jump condition $\Jump[]_t$ and initial set $\Init[]$, written as $\lb{j}(\Init,\Jump_t)$ and $\ub{j}(\Init,\Jump_t)$, is defined as below:
%            \begin{align*}
%                &\lb{j}(\Init[],\Jump[]_t)\,= \inf_{x_j\in\Reals}\left\{\forall (x_1,\!\cdots,\!x_{j-1},\!x_{j+1},\!\cdots,\!x_n,\!t), \Reach[](\Init)\to \Jump[]_t\right\} \\
%                &\ub{j}(\Init[],\Jump[]_t) = \sup_{x_j\in\Reals}\left\{\forall (x_1,\!\cdots,\!x_{j-1},\!x_{j+1},\!\cdots,\!x_n,\!t), \Reach[](\Init)\to \Jump[]_t\right\} \\
%            \end{align*} 
%        \end{definition}
%
%        We call the interval $[\lb{j}(\Init[],\Jump[]_t),\ub{j}(\Init[],\Jump[]_t)]$ as \emph{$j$-dimension jump condition} for trajectories staring from $\Init[]$ that should jump in time-relevant set $\Jump[]_t$. For clarity, we will denote this interval as $[\lb{j},\ub{j}]$ when there is no potential for confusion. Then we have the following lemma
%       \begin{lemma}
%           For a given convex initial set $\Init[]$ and its corresponding convex time-relevant jump condition $\Jump[]_t$, if the Cartesian product $\prod_{j=1}^{n}[\lb{j},\ub{j}]$ is non-empty, the trajectories staring from $\Init[]$ with $\Jump[]\Def\prod_{j=1}^{n}[\lb{j},\ub{j}]$ as jump condition will be a subset of the trajectories with $\Jump[]_t$ as time-relevant jump condition. 
%       \end{lemma}
%        \begin{proof}
%            Let's denote the set of trajectories with $\Jump[]$/$\Jump[]_t$ as jump condition as $\llangle\Jump[]\rrangle$/$\llangle\Jump[]\rrangle$ respectively. Because the trajectories in $\llangle\Jump[]\rrangle$ and $\llangle\Jump[]\rrangle$ are the same before switching happening, we only need to show that the trajectories in  $\llangle\Jump[]\rrangle$ after switching is in $\llangle\Jump[]\rrangle$.
%
%            Because $\Init[]$ and $\Jump[]_t$ is convex, $\Jump[]$ is also convex.\hscomment{ This statement needs more explanation } Thus for any state $\xx\in\Jump[]$, it satisfies 
%            \begin{align*}
%                \forall t,~\Reach[](\Init[])\to\Jump[]_t
%            \end{align*}
%            which is to say, for any trajectories staring from $\Init[]$, if it jumps at some point $\xx\in\Jump[]$ at time $t$, then the $(\xx,t)\in\Jump[]_t$, which is to say, this jump can also happen in $\Jump[]_t$, thus, the trajectories in  $\llangle\Jump[]\rrangle$ after switching is in $\llangle\Jump[]\rrangle$. 
%            
%        \end{proof}

    \subsection{Resolving  the Conflicts}

        Ideally, by identifying and combining all the $i$-switches guard conditions for each discrete transition into a single conjunctive condition, we can synthesize switched hybrid automata that meets the specified ST-RA formula. However, in more general scenarios, the $i$-switches guard conditions for the same edge might conflict, meaning their conjunction could be empty, as illustrated in \cref{exp:WTS-conflict}.

%        \begin{example}\label{exp:WTS-ideal}
%            Continuous to \cref{exp:WTS-HA}. Ideally, in mode $q_1$: 
%            \begin{itemize}
%                \item[1.] the trajectories staring from $\Init[q_1]^0=[0,1]$ should be jump-free, thus $\Jump[e_1]$ should satisfy the condition $cond(e_1)_0=(h<0\vee h>4)$ to avoid early switching,
%                \item[2.] the trajectories staring from $\Init[q_1]^1=(1,2]$ should include one jump before reaching the target set, thus $\Jump[e_1]$ should satisfy $cond(e_1)_1=(h\le 4\wedge h\ge 4)$,
%                \item[3.] the trajectories staring from $\Init[q_1]^2=(2,3]$ should include two jumps before reaching the target set, thus $\Jump[e_1]$ should satisfy $cond(e_1)_2=(h\le 4)$.
%            \end{itemize}
%            \hscommentinline{Figures to illustrate the following 3 condition}
%            Therefore, the viable jump condition for edge $e_1$ is $\Jump[e_1]=Cond(e_1)^0\wedge Cond(e_1)_1\wedge Cond(e_1)_2=(h\le4 \wedge h\ge 4)$. 
%           \end{example} 

        \begin{example}\label{exp:WTS-conflict}
            Continuing  \cref{exp:WTS-guard}, the conjunction of $i$-switches guard conditions 
            {\makeatletter
            \let\par\@@par
            \par\parshape0
            \everypar{}
            \begin{wrapfigure}{r}{0.42\textwidth}
		    \centering
            \vspace{-0.9cm}
            \begin{adjustbox}{max width = 1\linewidth}
		        \begin{tikzpicture}[font=\scriptsize]
		            \begin{groupplot}[ Axis Set, height = 3.7cm, group style={group size = 1 by 1, horizontal sep = 0.5cm}]
		                %%%X_{q_1}^1
                        \nextgroupplot[xmax=5, ymax=5.5,xlabel=$t$,ylabel=$h$,ytick={1,2,2.5,3,4,5}]
                        \addplot[name path = X1, draw = none] (0.7,0.7) node {$X_{q_1}^0$};
                        \addplot[name path = G1U, domain = {0:1}, draw = none] {x+1};
                        \addplot[name path = G1L, domain = {0:1}, draw = none] {0};
                        \addplot[fill=myorange!20]fill between[of=G1U and G1L, soft clip={domain=0:1}];
                        \addplot[name path = G2U, domain = {1:3}, draw = none] {x+1};
                        \addplot[name path = G2L, domain = {1:3}, draw = none] {x-1};
                        \addplot[fill=myorange!20]fill between[of=G2U and G2L, soft clip={domain=1:3}];
                        \addplot[name path = G3U, domain = {3:4}, draw = none] {4};
                        \addplot[name path = G3L, domain = {3:4}, draw = none] {x-1};
                        \addplot[fill=myorange!20]fill between[of=G3U and G3L, soft clip={domain=3:4}];
                        % Reachable set from [2,3]
                        %\node[coordinate, pin={[pin edge={Black}]80:{{$\Reach(\Init[q_2]^1)$}}}] at (axis cs:0.3, 3.3){};
                        \addplot[name path = reach3q1, domain = {0:1}, color = myorange, thick] {x+3};
                        \addplot[name path = reach2q1, domain = {0:2}, color = myorange, thick] {x+2};
                        \addplot[name path = reach3q2, domain = {1:4}, color = mygreen, thick] {-x+5};
                        \addplot[name path = reach2q2, domain = {2:4}, color = mygreen, thick] {-x+6};
                        % t-eleminate result
                        \addplot[name path = guardUB, domain = {0:3.5}, color=mygray,thick] {3};
                        \addplot[name path = guardLB, domain = {0:3.5}, color=mygray,thick] {2.5};
                        
                        % The STL specification
		                \addplot[name path = Phi2Up,  domain = {3:4}, color=myblue] {5};% node [right] {$\phi_2$};
		                \addplot[name path = Phi2Low, domain = {3:4}, color=myblue] {3};
                        \addplot[name path = Phi1, domain = {0:4}, color = myred] {4};% node [right] {$\phi_1$};
                        % Dash line
		                \draw[dashed] ($(axis cs:3,\pgfkeysvalueof{/pgfplots/ymax})!{1/11}!(axis cs:3,\pgfkeysvalueof{/pgfplots/ymin})$) -- (axis cs:3,\pgfkeysvalueof{/pgfplots/ymin});
		                \draw[dashed] ($(axis cs:4,\pgfkeysvalueof{/pgfplots/ymax})!{1/11}!(axis cs:4,\pgfkeysvalueof{/pgfplots/ymin})$) -- (axis cs:4,\pgfkeysvalueof{/pgfplots/ymin});

		                \addplot[name path = NewInit,  domain = {1:2}, color=Purple, very thick] {4};
                    \end{groupplot}
		        \end{tikzpicture}
            \end{adjustbox}
            \vspace{-0.7cm}
            \caption{Conflict in $G(q_2,q_1)$}
            \label{fig:t-conflict}
            \end{wrapfigure}
            \noindent
            of $e_1=(q_1,q_2)$ can successfully yield $G(e_1) = (h \leq 4 \wedge h \geq 4)$. Consequently, for executions beginning from $\Init[q_1]^2=(2,3]$, the first switch occurs at $h=4$, facilitating the control mode transition from $q_1$ to $q_2$. This switch is visually depicted in \cref{fig:t-conflict} by the change in color of the reachable set boundary from orange ($q_1$) to green ($q_2$). 

            \par}%
            After discrete transition $e_1$, the conjunction of $\Reach(\Init[q_1]^2)$ and $G(e_1)$, i.e., the purple line segment in \cref{fig:t-conflict}, will be added to $\Init[q_2]^1$. Such operation is to ensure that the execution after switch will still maintain a feasible guard condition. However, this additional initial condition will lead to a conflict, as it requests $G(q_2,q_1)^0$ satisfying $(2.5\leq h\leq 3)$, while the previous example in \cref{exp:WTS-guard} requests that $(1.5\leq h\leq 2)$.
            \qedT
        \end{example}

        Hence, to avoid such conflicts, specific $i$-switches guard conditions may need to be expanded. For instance, the constraint $(1.5 \leq h \leq 2)$ in \cref{exp:WTS-guard} can be expanded to $(1.5 \leq h \leq 2.5)$ by substituting the left part of \cref{eq:eliminate-exp} with $X_{q_1}^1$, resulting in a feasible $t$-eliminated outcome: $G(q_2,q_1) = (h \geq 2.5 \wedge h \leq 2.5)$. 
        
        In a logical formula ($A\!\!\implies\!\! B$), constraining $A$ or expanding $B$ enhances the satisfiability of the formula. Thus, \cref{eq:t-irr-formula} indicates two ways to expand $G(q,q')^i$:
        %\simoncomment{might need some explannation here}:
        \begin{enumerate}[label=(\roman*)]
            \item Constrain the size of the initial set $\Init[q]^{i+1}$.
            \item Expand the state-time set $X_{q'}^i$. 
        \end{enumerate}

        By constraining the size of the initial set $\Init[q]^i$, a correspondingly smaller reachable set is achieved, facilitating the accommodation of a larger $i$-switches guard condition. In more extreme cases, certain initial sets can be omitted to prevent conflicts. This process trims the set of executions of switched hybrid automata, yet it maintains the satisfaction of the switched hybrid automata with respect to $\varphi$.

        Considering that removing initial sets may reduce the number of executions for switched hybrid automata, we prefer the second method involving the expansion of $X_{q'}^i$. However, since this process essentially enlarges the set of executions of the switched hybrid system, careful consideration is needed when enlarging $X_{q'}^i$. The following lemma provides a proper enlargement strategy
        \begin{restatable}{lemma}
        {restateCortEnlarge}\label{lm:cort-enlarge}
            Given $\{\Init[q]^i\}_{q\in Q}$, $\{X_q^i\}_{q\in Q}$ calculated by \cref{alg:time-relevant-syn}, and ST-RA formula $\varphi$, executions $\xx$ starting from $\Init[q]^{i+1}$ with the first switch happens at $(\xx(\tau),\tau)\in X_{q'}^{i+l}$, $l\in\PosNats$, can also satisfy $\varphi$.
        \end{restatable}
  \oomit{     \begin{proof}
            Indeed, we only need to prove the lemma for $k=1$, and the result for larger $k$ follows inductively. From \cref{cor:all_initial}, we know that $X_{q'}^i \subseteq X_{q'}^{i+1}$. If the first switch for executions starting from $\Init[q]^{i+1}$ occurs at $(\xx(\tau),\tau)\in X_{q'}^i \subseteq G_t(q,q')^{i+1}$, satisfaction of $\varphi$ is straightforward by \cref{thm:induc_state-time_set}. If the first switch occurs at $(\xx(\tau),\tau)\in X_{q'}^{i+1} \setminus X_{q'}^i$, according to \cref{def:state-time_set}, signals starting from $(\xx(\tau),\tau)$ will satisfy $\varphi$ within additional $i+1$ times of switches. Thus, the lemma is proved.
            \qed 
        \end{proof} }
        
        %Due to the nondeterministic nature of switches in hybrid automata upon satisfying guard conditions and domains, 
        As elucidated in \cite{henzinger1996theory}, in hybrid automata, a transition to the next mode may or may not occur when both the guard condition and the current mode's domain are satisfied. However, a switch becomes deterministic if the domain of the current mode is violated while the guard condition remains satisfied. Therefore, to ensure a predictable switch upon entering a calculated guard condition, it's crucial to define the domain's boundary as the specific segment of the guard conditions' boundary where the execution is expected to exit. This segment is referred to as the ``exit boundary'' of the guard conditions
        %As discussed in \cite{henzinger1996theory}, an execution of hybrid automata might or might not switch to the next mode when both the guard condition and the mode's domain are satisfied, but the switch will deterministically happen if the current mode's domain is violation but the guard condition is still satisfied. 
        %Therefore, to ensure that the switch will eventually happen when it enter a guard condition we calculated, we need to defined the boundary of the domain as the segment of boundary of guard conditions where the execution will leave these boundary, we call it the "existing boundary" of guard consitions.
        %
        %To ensure that each discrete transition happens immediately if its  guard holds, the domain of each mode should be defined as the the complementary of the union of the guards of these outward edges from it.\simoncomment{revise last sentence, hard to understand} 
        %``existing boundary" of the guard conditions - segment of the guard conditions' boundary where the execution is expected to exit.

        To determine the ``exiting boundary'', we check the sign of the inner product between the direction of the boundary and the partial derivatives of vector fields. Formally, for a mode $q$ with a flow condition defined by $\dot{\xx}= f_q(\xx)$ and a guard condition defined by a Boolean combination of linear inequalities in the form $b^T x \ge c$, the boundary of the domain is defined by those inequalities that satisfy:% the following condition:
        \begin{align}\label{eq:inv-justif}
            b \cdot \frac{\partial f_q}{\partial \xx} < 0.
        \end{align}

\begin{algorithm}[t]
            \caption{Switch Logic Controller Synthesize Algorithm}
            \label{alg:switch-syn}
            \begin{algorithmic}[1] % The number tells where the line numbering should start
                \Require $\{X_q^i\}_{q\in Q}$ and $\{\Init[q]^i\}_{q\in Q}^k$ for $i=0,1,\cdots,k$ 
                \Ensure $G(e)$ for $e\in E$, $\Dom[q]$ for $q\in Q$
                %\Procedure{Euclid}{$a,b$} \Comment{The g.c.d. of a and b}
                \While {$E$ is not empty}
                    \State Pop $e=(q,q')$ from $E$
                    \Repeat \label{alg2:guard-start}
                        \State Calculate $i$-switches guard condition $G(e)^i$ for $i=0,\cdots,k$  \Comment{\cref{eq:t-irr-formula}}
                        \State Expand $X_{q'}^i$ to $X_{q'}^{j}$, $j>i$ or constrain $\Init[q]^{i+1}$ to solve conflicts \label{alg2:sol-conflict}
                            %\State \textbf{Break}
                    \Until{there is no conflict}\label{alg2:guard-end}
                    \State $G(e)\gets \wedge_{i=0}^k G(e)^i$
                    \State Add $ G(e)\wedge\Reach(\Init[q]^i)$ to $\Init[q']^{i-1}$ for $i=1,\cdots,k$ \label{alg2:add-init}
                    \State Add $e=(q',\text{post-mode of }q')$ to $E$ if $\Init[q']^{i-1}$ is enlarged for some $i$ \label{alg2:add-edge}
                \EndWhile
                \State $\Init[q] \gets \vee_i\Init[q]^i[t\repl 0]$
                \State Define the domain $\Dom[q]$          \Comment{ \cref{eq:inv-justif}}  
                %\Return $G(e),\Dom[q]$ 
                %\EndProcedure
            \end{algorithmic}
        \end{algorithm}



        We summarize the overall idea as outlined in \cref{alg:switch-syn}. The switched hybrid automata satisfying an ST-RA formula $\varphi$ are synthesized based on the results obtained from \cref{alg:time-relevant-syn}, with an additional discrete transition set $E$. For each edge $e=(q,q')\in E$, the algorithm initially attempts to find a feasible guard condition (lines \ref{alg2:guard-start} - \ref{alg2:guard-end}). Once a guard condition is identified, the intersection of the boundary condition and $\Reach(\Init[q]^i)$ is added to $\Init[q']^{i-1}$ (line \ref{alg2:add-init}). This ensures that the execution, after switching to $q'$, will still maintain a feasible guard condition. As the initial set is renewed, the corresponding $i$-switches guard conditions will be recalculated by re-adding them to $E$ (line \ref{alg2:add-edge}). Finally, if the procedure terminated, the initial set and domain will be synthesized.

        Given that the procedure to resolve conflicts (as indicated in line \ref{alg2:sol-conflict}) is fundamentally heuristic in nature, \cref{alg:switch-syn} is correct yet not complete. The correctness of \cref{alg:switch-syn} is affirmed by \cref{thm:cort-switch-syn}.

%        As the procedure of resolve the conflicts (line \ref{alg2:sol-conflict}) is essentially heuristic, \cref{alg:switch-syn} is correct but not complete. The correctness of \cref{alg:switch-syn} is provided by \cref{thm:cort-switch-syn}.
        
        \begin{restatable}{theorem}
        {restateCortSwitchSyn}\label{thm:cort-switch-syn}
            If \cref{alg:switch-syn} terminate, all  executions of the synthesized switched hybrid automaton $\HyAuto$ satisfy the given ST-RA formula $\varphi$.
        \end{restatable}
   \oomit{     \begin{proof}
            \cref{thm:leastest-jump-times} ensures that the system before $t$-elimination satisfying $\varphi$. As \cref{lm:cort-enlarge} ensure the correctness of the conflicts resolve process, the correctness of \cref{alg:switch-syn} is proved. 
            \qed
        \end{proof} }
%    \begin{remark}
%        We heuristically permit a single jump in the trajectory originating from $\Init[]^0$ initially, thereby averting the scenario of dismissing numerous viable jump conditions due to the necessity for the trajectory commencing from $\Init[]_0$ to remain jump-free.
%    \end{remark}
%    \begin{theorem}
%       For a given mode $q$ and jumping times $i$, if the Cartesian product $\prod_{j=1}^{n}[\lb{j}(q,i),\ub{j}(q,i)]$ of the $j$-dimension $i$-times jump condition is non-empty, the trajectories staring from $\Init[q]^i$ with $\prod_{j=1}^{n}[\lb{j}(q,i),+\infty)$ as jump condition and $\prod_{j=1}^{n}(-\infty,\ub{j}(q,i)]$ as invariant condition will satisfy the given STL specification $\varphi$ in $i$ times jump.
%    \end{theorem}
            

        
    

==> tikzkey.tex <==
\RequirePackage{tikz}
\RequirePackage{pgfplots}

\usetikzlibrary{
	cd,
	math,
	decorations.markings,
	decorations.pathreplacing,
	positioning,
	arrows.meta,
	circuits.logic.US,
	shapes,
	calc,
	fit,
	quotes,
  scopes,
  patterns,
  backgrounds}

\usepgfplotslibrary{groupplots, fillbetween}


\tikzset{
        oriented WD/.style={%everything after equals replaces "oriented WD" in key.
           %every to/.style={out=0,in=180,draw},
           label/.style={
              font=\everymath\expandafter{\the\everymath\scriptstyle},
              inner sep=0pt,
              node distance=2pt and -2pt},
           semithick,
           node distance=1 and 1,
           decoration={markings, mark=at position \stringdecpos with \stringdec},
           ar/.style={postaction={decorate}},
           execute at begin picture={\tikzset{
              x=\bbx, y=\bby,
              every fit/.style={inner xsep=\bbx, inner ysep=\bby}}}
           },
        string decoration/.store in=\stringdec,
        string decoration={\arrow{stealth};},
        string decoration pos/.store in=\stringdecpos,
        string decoration pos=.7,
        bbx/.store in=\bbx,
        bbx = 1.5cm,
        bby/.store in=\bby,
        bby = 1.5ex,
        bb port sep/.store in=\bbportsep,
        bb port sep=1.5,
        % bb wire sep/.store in=\bbwiresep,
        % bb wire sep=1.75ex,
        bb port length/.store in=\bbportlen,
        bb port length=4pt,
        bb penetrate/.store in=\bbpenetrate,
        bb penetrate=0,
        bb min width/.store in=\bbminwidth,
        bb min width=1cm,
        bb rounded corners/.store in=\bbcorners,
        bb rounded corners=2pt,
        bb small/.style={bb port sep=1, bb port length=2.5pt, bbx=.4cm, bb min width=.4cm, 
   bby=.7ex},
            bb medium/.style={bb port sep=1, bb port length=2.5pt, bbx=.4cm, bb min width=.4cm, 
   bby=.9ex},
        bb/.code 2 args={%When you see this key, run the code below:
           \pgfmathsetlengthmacro{\bbheight}{\bbportsep * (max(#1,#2)+1) * \bby}
           \pgfkeysalso{draw,minimum height=\bbheight,minimum width=\bbminwidth,outer 
   sep=0pt,
              rounded corners=\bbcorners,thick,
              prefix after command={\pgfextra{\let\fixname\tikzlastnode}},
              append after command={\pgfextra{\draw
                 \ifnum #1=0{} \else foreach \i in {1,...,#1} {
%                    ($(\fixname.north west)!{\i/(#1+1)}!(\fixname.south west)$) +(-\bbportlen,0) coordinate (\fixname_in\i) -- +(\bbpenetrate,0) coordinate (\fixname_in\i')}\fi 
                    ($(\fixname.north west)!{\i/(#1+1)}!(\fixname.south west)$) +(0,0) coordinate (\fixname_in\i) -- +(\bbpenetrate,0) coordinate (\fixname_in\i')}\fi 
     %Define the endpoints of tickmarks
                 \ifnum #2=0{} \else foreach \i in {1,...,#2} {
%                    ($(\fixname.north east)!{\i/(#2+1)}!(\fixname.south east)$) +(-\bbpenetrate,0) coordinate (\fixname_out\i') -- +(\bbportlen,0) coordinate (\fixname_out\i)}\fi;
                    ($(\fixname.north east)!{\i/(#2+1)}!(\fixname.south east)$) +(-\bbpenetrate,0) coordinate (\fixname_out\i') -- +(0,0) coordinate (\fixname_out\i)}\fi;
              }}}
        },
        bb name/.style={append after command={\pgfextra{\node[anchor=north] at 
   (\fixname.north) {#1};}}}     
}

\pgfplotsset{
  Axis Set/.style = {
    axis lines=middle,
		every axis y label/.style={
			at={(ticklabel* cs:1)},
			anchor=south,
		},
		%			footnotesize,
		width = 6.5cm, %% As big as this example can be without spilling over onto the next slide
		height = 4cm, %% ditto
		%			ticks = none,
		xtick = {1,2,3,4},
    %ytick = {1,2,3,4,5},
    xmin = 0, 
    ymin = 0
  }
}
